Using Natural Language Explanations to Improve Robustness of In-context Learning

Recent studies demonstrated that large language models (LLMs) can excel in many tasks via in-context learning (ICL). However, recent works show that ICL-prompted models tend to produce inaccurate results when presented with adversarial inputs. In this work, we investigate whether augmenting ICL with natural language explanations (NLEs) improves the robustness of LLMs on adversarial datasets covering natural language inference and paraphrasing identification. We prompt LLMs with a small set of human-generated NLEs to produce further NLEs, yielding more accurate results than both a zero-shot-ICL setting and using only human-generated NLEs. Our results on five popular LLMs (GPT3.5-turbo, Llama2, Vicuna, Zephyr, and Mistral) show that our approach yields over 6% improvement over baseline approaches for eight adversarial datasets: HANS, ISCS, NaN, ST, PICD, PISP, ANLI, and PAWS. Furthermore, previous studies have demonstrated that prompt selection strategies significantly enhance ICL on in-distribution test sets. However, our findings reveal that these strategies do not match the efficacy of our approach for robustness evaluations, resulting in an accuracy drop of 8% compared to the proposed approach.

==> tab-extractable.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{cccc}
    \toprule
     \multirow{2}{*}{\textbf{Data}} &  \multicolumn{3}{c}{\textbf{Models}}\\
     \cmidrule(lr){2-4}
     &\textbf{ LLaMA}& \textbf{Vicuna}&\textbf{ChatGPT}  \\
    \midrule
HANS &0.0  & 0.0 &0.0 \\
ISCS  &0.0 & 0.0  &0.0  \\
NaN  & 0.0& 0.0 &0.0  \\
ST  &0.0 & 0.0  &0.0   \\
PICD & 0.0& 0.0  & 0.0	\\
PISP & 0.0& 0.0  & 0.0	 \\
ANLI (R1) & 0.0 & 0.0 & 0.0  \\
ANLI (R2) &  0.0 &  0.0&  0.0 \\
ANLI (R3) & 0.0 & 0.0 &  0.0  \\						
    \bottomrule
    \end{tabular}
    \caption{Fraction of extractable instances of each dataset based on LLaMA, Vicuna, and ChatGPT.}
    \label{tab:extractable}
\end{table}

==> tab-full.tex <==
% \begin{table*}[!th]
%     \centering
%     \small
%     \begin{tabular}{clccccccc| c}
%     \toprule
%     \textbf{Models}& \textbf{Methods}& \textbf{HANS} & \textbf{ISCS}& \textbf{NaN}	& \textbf{ST} & \textbf{PICD} & \textbf{PISP} & \textbf{ANLI (R1/R2/R3)} & \textbf{Avg.}\\
%     \midrule
%    \multirow{4}{*}{{\rotatebox[origin=c]{90}{\textbf{OPT}}}}& \caseone & 50.4 & 34.6 & \textbf{37.7} & 36.5 & 33.9 & \textbf{53.0} &	32.4 / 33.1 /	34.6 & 38.5\\
%    &\casetwo& 50.0	& 34.8	& 37.4	& \textbf{37.6}	& 36.2& 	52.8	&32.5 / 32.9 / 34.4	& \textbf{38.7} \\
%    &\casefour & 50.2	& 34.7	& 30.4	& 34.9	& 34.9	& 34.5	& 30.1 / \textbf{34.6} / 33.7 & 35.3\\
%    &\casethree & \textbf{52.8} &	\textbf{36.6}	&28.7	&34.7&	\textbf{37.5}	&42.3&	\textbf{34.8} / 34.2 / \textbf{35.9} & 37.5\\
%    \midrule
% \multirow{4}{*}{{\rotatebox[origin=c]{90}{\textbf{OPT-IML}}}} &\caseone & \textbf{57.9}& 34.7	& \textbf{41.9}	& 40.2	& 46.8	& 51.5 & 37.2 / 35.7 / 36.6 & 42.5\\
% &\casetwo &57.6 & 40.4	& 40.2	& \textbf{45.0}	& \textbf{53.1}	& \textbf{57.8} & 39.8	/ 36.9 / \textbf{37.6} & \textbf{45.4}\\
% &\casefour&55.0 & 40.4	& 35.2	& 41.6	& 43.8	& 53.9 & 35.4 / 32.6 / 33.1 & 41.2\\
% &\casethree &53.2 & \textbf{40.6}	& 32.2	& 41.0	& 41.2	& 48.1 & \textbf{43.0} / \textbf{38.5} / 36.2 & 41.6\\
% \midrule
% \multirow{4}{*}{{\rotatebox[origin=c]{90}{\textbf{LLaMA}}}}&\caseone& 59.7 & 53.8 & 51.7 & 52.7 & \textbf{66.0} & 42.1	& 49.2 / 43.5	/ 41.5	& 51.1 \\
% &\casetwo& \textbf{62.3}	& 55.3	& 57.7& 52.8 & 	51.8	& 47.3	& 48.1 /	44.6 / 43.5	 & 51.5\\
% &\casefour& 55.5 &	52.4	& 54.4	& 49.6	& 45.1	& 30.5	& 54.3	/ 47.5	/ 46.6	& 48.4 \\
% &\casethree& 58.9	& \textbf{57.7}	& \textbf{62.8}	& \textbf{58.3}	& 60.9	& \textbf{52.8}	& \textbf{60.5} / \textbf{49.3} /  \textbf{50.8}	 & \textbf{56.9} \\
% \midrule
% \multirow{4}{*}{{\rotatebox[origin=c]{90}{\textbf{Vicuna}}}}&\caseone& 69.4	&62.7	& 61.4	& 58.7	& \textbf{67.1}	& 50.9 & 55.2 / 48.8 / 46.0 & 57.8\\
% &\casetwo& 62.9	& 60.9	& 64.2	& 57.3	& 63.7	& 55.0	& 57.0 / 48.9 / 38.8	& 56.5  \\
% &\casefour & 61.4 & 64.9	& 60.2	& 61.7	& 57.9	& 51.8 & 51.7 / 47.9 / 49.4	 & 56.3 \\
% &\casethree  & \textbf{74.5}	& \textbf{65.5}	& \textbf{66.3}	& \textbf{64.8}	& 61.6	& \textbf{65.9}	& \textbf{64.9} / \textbf{55.5} / \textbf{52.0} & \textbf{63.4} \\
% \midrule
% \multirow{4}{*}{{\rotatebox[origin=c]{90}{\textbf{ChatGPT}}}} &\caseone&  72.4& 64.4	& 70.0 & 62.1	&64.0 & 51.2 & 62.4 / 51.7 / 54.4  & 61.4\\
% & \casetwo & 71.0	& 69.0 & 70.5 & 65.7 & 72.7 & 59.3 & 67.2 / 55.1 / 56.9 & 65.3\\
% &\casefour  & 71.6& 68.4	& 70.2	& 67.6	& 67.7	& 61.7	& 67.9	/ \textbf{56.4}	/ \textbf{56.9} & 65.4\\
% & \casethree & \textbf{76.0} & \textbf{74.9} & \textbf{73.1} & \textbf{73.3} & \textbf{76.9} & \textbf{75.5}	& \textbf{68.5} / 54.4 / 55.9 & \textbf{69.8}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Accuracy of multiple LLMs using (1) standard ICL without NLEs, (2) \xicl with human-written NLEs: \casetwo, (3) \xicl with ChatGPT-generated NLEs in a zero-shot scenario: \casefour, (4)  \xicl with ChatGPT-generated NLEs in a few-shot scenario: \casethree. The best performance for each task within a model is shown in \textbf{bold}. \xh{add std and statistical test}}
%     \label{tab:main}
% \end{table*}

\begin{table*}[!th]
    \centering
    \scalebox{0.84}{
    \begin{tabular}{clccccccc| c}
    \toprule
    \textbf{Models}& \textbf{Methods}& \textbf{HANS} & \textbf{ISCS}& \textbf{NaN}	& \textbf{ST} & \textbf{PICD} & \textbf{PISP} & \textbf{ANLI (R1/R2/R3)} & \textbf{Avg.}\\
    \midrule
   \multirow{8}{*}{{\rotatebox[origin=c]{90}{\textbf{OPT}}}}& \caseone & 50.4\ \ \ & 34.6\ \ \ & \textbf{37.7}\ \ \ & 36.5\ \ \ & 33.9\ \ \ & \textbf{53.0}\ \ \ &	32.4\ \ \ / 33.1\ \ \ /	34.6\ \ \ & 38.5 \vspace{-0.15cm}\\
   % \vspace{-0.1cm}
    & & \std{0.1}& \std{0.7} & \std{0.2} & \std{0.2} & \std{0.4} & \std{2.3} & \threestd{0.7}{0.1}{0.7}\\
% \std{0.7} / \std{0.1} / \std{0.1} \\
   &\casetwo& 50.0\ \ \ & 34.8\ \ \ & 37.4\ \ \ & \textbf{37.6}$^\triangledown$	& 36.2$^\triangledown$& 	52.8\ \ \ &32.5\ \ \ / 32.9\ \ \ / 34.4\ \ \ & \textbf{38.7} \vspace{-0.15cm}\\
 & & \std{0.8} & \std{1.0} & \std{0.8} & \std{0.6} & \std{1.8} & \std{1.3} & \threestd{0.7}{0.3}{0.2} \\
   &\casefour & 50.2\ \ \ & 34.7\ \ \ & 30.4\ \ \ & 34.9\ \ \ & 34.9\ \ \ & 34.5\ \ \ & 30.1\ \ \ / \textbf{34.6}\ \ \ / 33.7\ \ \ & 35.3 \vspace{-0.15cm}\\
 && \std{1.4} &\std{4.0} & \std{12.3} & \std{5.2} & \std{2.4} & \std{11.1} & \threestd{2.9}{2.1}{2.4}\\
   &\casethree & \textbf{52.8}\ \ \ &	\textbf{36.6}\ \ \ &28.7\ \ \ &34.7\ \ \ & \textbf{37.5}$^\triangledown$&42.3\ \ \ &	\textbf{34.8}\ \ \ / 34.2$^\triangledown$ / \textbf{35.9}$^\triangledown$ & 37.5 \vspace{-0.15cm}\\
    & &  \std{3.1} & \std{3.9} & \std{10.6}	& \std{3.3} & \std{2.6} & \std{10.5}	& \threestd{2.8}{0.8}{0.9} \\
   \midrule
\multirow{8}{*}{{\rotatebox[origin=c]{90}{\textbf{OPT-IML}}}} &\caseone & \textbf{57.9}\ \ \ & 34.7\ \ \ & \textbf{41.9}\ \ \ & 40.2\ \ \ & 46.8\ \ \ & 51.5\ \ \ & 37.2\ \ \ / 35.7\ \ \ / 36.6\ \ \ & 42.5 \vspace{-0.15cm}\\
& & \std{2.5} & \std{1.4} &	\std{6.1} & \std{3.9} & \std{3.8} & \std{3.0}	& \threestd{2.5}{1.2}{1.8}\\
&\casetwo &57.6\ \ \ & 40.4$^\blacktriangledown$	& 40.2\ \ \ & \textbf{45.0}$^\triangledown$	& \textbf{53.1}$^\triangledown$	& \textbf{57.8}$^\triangledown$ & 39.8\ \ \ / 36.9\ \ \ / \textbf{37.6}\ \ \ & \textbf{45.4} \vspace{-0.15cm}\\
& & \std{2.4} & \std{3.0} & \std{1.9} & \std{3.2} & \std{5.7} & \std{4.1} & \threestd{2.3}{0.5}{0.5}\\
&\casefour&55.0\ \ \ & 40.4$^\triangledown$	& 35.2\ \ \ & 41.6\ \ \ & 43.8\ \ \ & 53.9\ \ \ & 35.4\ \ \ / 32.6\ \ \ / 33.1\ \ \ & 41.2 \vspace{-0.15cm}\\
& & \std{7.5} & \std{4.0} & \std{10.8} & \std{6.9} & \std{6.2}  & \std{7.8} & \threestd{7.5}{5.5}{5.7} \\
&\casethree &53.2\ \ \ & \textbf{40.6}$^\blacktriangledown$	& 32.2\ \ \ & 41.0\ \ \ & 41.2\ \ \ & 48.1\ \ \ & \textbf{43.0}$^\triangledown$ / \textbf{38.5}$^\triangledown$ / 36.2\ \ \ & 41.6 \vspace{-0.15cm}\\
&& \std{2.6} & \std{3.5} & \std{8.1} & \std{2.4} & \std{3.5} & \std{9.2} & \threestd{3.2}{1.1}{0.8} \\
\midrule
\multirow{8}{*}{{\rotatebox[origin=c]{90}{\textbf{LLaMA 30B}}}}&\caseone& 59.7\ \ \ & 53.8\ \ \ & 51.7\ \ \ & 52.7\ \ \ & \textbf{66.0}\ \ \ & 42.1\ \ \ & 49.2\ \ \ / 43.5\ \ \ / 41.5\ \ \ & 51.1 \vspace{-0.15cm}\\
&& \std{3.4} & \std{1.6}	& \std{2.3} & \std{4.4} & \std{3.0} & \std{7.3}& \threestd{3.6}{2.1}{3.2} \\
&\casetwo& \textbf{62.3}\ \ \ & 55.3\ \ \ & 57.7$^\triangledown$& 52.8\ \ \ &51.8\ \ \ & 47.3\ \ \ & 48.1\ \ \ / 44.6\ \ \ / 43.5\ \ \ & 51.5 \vspace{-0.15cm}\\
&& \std{4.6}	& \std{4.4}	& \std{3.3}	& \std{3.9} & \std{2.3} & \std{5.1} & \threestd{4.3}{2.1}{1.3}\\
&\casefour& 55.5\ \ \  & 52.4\ \ \ & 54.4\ \ \ & 49.6\ \ \ & 45.1\ \ \ & 30.5\ \ \ & 54.3$^\triangledown$ / 47.5$^\triangledown$ / 46.6$^\triangledown$& 48.4 \vspace{-0.15cm}\\
&&\std{6.3} & \std{6.0}	& \std{5.4} & \std{5.4} & \std{8.5} & \std{8.7} & \threestd{0.8}{0.7}{0.9} \\
&\casethree& 58.9\ \ \ & \textbf{57.7}$^\blacktriangledown$	& \textbf{62.8}$^\blacktriangledown$ & \textbf{58.3}$^\triangledown$	& 60.9\ \ \ & \textbf{52.8}\ \ \ & \textbf{60.5}$^\blacktriangledown$ / \textbf{49.3}$^\triangledown$ /  \textbf{50.8}$^\triangledown$& \textbf{56.9} \vspace{-0.15cm}\\
&& \std{8.5} & \std{1.2} & \std{3.2} & \std{3.7} &\std{6.5} & \std{5.9} & \threestd{1.1}{2.2}{1.6} \\
\midrule
\multirow{8}{*}{{\rotatebox[origin=c]{90}{\textbf{Vicuna}}}}&\caseone& 69.4\ \ \ &62.7\ \ \ & 61.4\ \ \ & 58.7\ \ \ & \textbf{67.1}\ \ \ & 50.9\ \ \ & 55.2\ \ \ / 48.8\ \ \ / 46.0\ \ \ & 57.8 \vspace{-0.15cm}\\
&&\std{1.2}	& \std{0.9} & \std{3.5} & \std{0.8} & \std{1.6} & \std{1.3} & \threestd{1.9}{1.8}{4.0}\\
&\casetwo& 62.9\ \ \ & 60.9\ \ \ & 64.2\ \ \ & 57.3\ \ \ & 63.7\ \ \ & 55.0\ \ \ & 57.0\ \ \ / 48.9\ \ \ / 38.8\ \ \ & 56.5  \vspace{-0.15cm}\\
&& \std{3.7}	 & \std{2.2} & \std{1.2} & \std{2.0} & \std{7.2} & \std{5.8} & \threestd{2.8}{3.1}{8.2} \\
&\casefour & 61.4\ \ \ & 64.9\ \ \ & 60.2\ \ \ & 61.7\ \ \ & 57.9\ \ \ & 51.8\ \ \ & 51.7\ \ \ / 47.9\ \ \ / 49.4	\ \ \ & 56.3 \vspace{-0.15cm}\\
&& \std{7.7} & \std{2.3} & \std{4.0} & \std{3.1} & \std{8.7} & \std{8.7} & \threestd{5.8}{4.6}{0.5} \\
&\casethree  & \textbf{74.5}$^\triangledown$	& \textbf{65.5}$^\triangledown$	& \textbf{66.3}$^\triangledown$	& \textbf{64.8}$^\blacktriangledown$	& 61.6\ \ \ & \textbf{65.9}$^\blacktriangledown$	& \textbf{64.9}$^\blacktriangledown$ / \textbf{55.5}$^\triangledown$ / \textbf{52.0}$^\triangledown$ & \textbf{63.4} \vspace{-0.15cm}\\
&& \std{4.4}	& \std{1.6} & \std{1.1} & \std{1.8} & \std{8.9} & \std{4.7} & \threestd{1.3}{1.0}{1.7}\\
\midrule
\multirow{7}{*}{{\rotatebox[origin=c]{90}{\textbf{ChatGPT}}}} &\caseone&  72.4\ \ \ & 64.4\ \ \  	& 70.0\ \ \  & 62.1\ \ \ &64.0\ \ \   & 51.2\ \ \   & 62.4\ \ \   / 51.7\ \ \   / 54.4\ \ \    & 61.4   \vspace{-0.15cm}\\
& & \std{0.6}	& \std{0.9} & \std{0.8} & \std{1.6} & \std{3.1} & \std{0.4} & \threestd{3.2}{0.9}{2.1} \\
& \casetwo & 71.0\ \ \  & 69.0$^\triangledown$ & 70.5\ \ \  & 65.7$^\triangledown$ & 72.7$^\blacktriangledown$& 59.3$^\triangledown$ & 67.2\ \ \ / 55.1$^\blacktriangledown$ / 56.9\ \ \   & 65.3  \vspace{-0.15cm}\\
&& \std{1.7}	&\std{1.2} & \std{2.2}& \std{1.0} & \std{1.3} & \std{1.9}	& \threestd{3.8}{0.2}{3.0} \\
&\casefour  & 71.6\ \ \  & 68.4$^\triangledown$	& 70.2\ \ \ 	& 67.6$^\triangledown$	& 67.7$^\triangledown$	& 61.7$^\blacktriangledown$	& 67.9$^\triangledown$	/ \textbf{56.4}$^\triangledown$	/ \textbf{56.9}$^\triangledown$ & 65.4 \vspace{-0.15cm}\\
 & & \std{0.8}	& \std{0.3}	& \std{0.0}	&\std{1.3} & \std{4.1} & \std{1.9}	& \threestd{2.6}{1.7}{1.7} \\
& \casethree & \textbf{76.0}$^\blacktriangledown$ & \textbf{74.9}$^\blacktriangledown$& \textbf{73.1}$^\blacktriangledown$ & \textbf{73.3}$^\blacktriangledown$ & \textbf{76.9}$^\blacktriangledown$ & \textbf{75.5}$^\blacktriangledown$	& \textbf{68.5}$^\blacktriangledown$ / 54.4$^\triangledown$ / 55.9$^\triangledown$ & \textbf{69.8} \vspace{-0.15cm}\\
&& \std{2.0} & \std{0.1} & \std{1.4} & \std{0.4} & \std{0.4} & \std{3.0} & \threestd{1.8}{2.4}{1.3} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Accuracy of multiple LLMs using (1) standard ICL without NLEs, (2) \xicl with human-written NLEs: \casetwo, (3) \xicl with ChatGPT-generated NLEs in a zero-shot scenario: \casefour, (4)  \xicl with ChatGPT-generated NLEs in a few-shot scenario: \casethree. The best performance for each task within a model is shown in \textbf{bold}. Significance testing was assessed via an unequal variances \textit{t}-test in comparison with \caseone: $\blacktriangledown$ (resp. $\triangledown$) represents a \textit{p}-value lower than $10^{\texttt{-}3}$ (resp. $10^{\texttt{-}1}$).}
    \label{tab:main}
    % \vspace{-0.5cm}
\end{table*}

==> tab-len-nle.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|ccc}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
